Pulser: Fast Congestion Response using Explicit Incast Notifications for Datacenter Networks

Datacenter applications frequently cause incast congestion, which degrades both flow completion times of short flows and throughput of long flows. Without isolating incast, existing congestion control schemes (e.g., DCTCP) rely on existing ECN signal to react to general congestion, and they lose performance due to their slow, cautious, and inaccurate reaction to incast. We propose to isolate incast using Explicit Incast Notifications (EIN) that are generated by switches, similar to ECN. Our incast detection is fast and accurate. Further, we present our congestion control scheme, called Pulser, which drastically backs off during incast based on EIN, but restores sending rate once incast ends. Our real experiments and ns-3 simulations show that Pulser outperforms prior schemes, DCTCP and ICTCP, in both flow completion times and throughput.

==> Makefile <==
PACKAGE=acmart

SAMPLES = \
	sample-sigconf.tex 


PDF = ${SAMPLES:%.tex=%.pdf} 

all:  ${PDF}

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf.pdf: samplebody-conf.tex

clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

